The SM and NLO Multileg and SM MC Working Groups: Summary Report

The 2011 Les Houches workshop was the first to confront LHC data. In the two years since the previous workshop there have been significant advances in both soft and hard QCD, particularly in the areas of multi-leg NLO calculations, the inclusion of those NLO calculations into parton shower Monte Carlos, and the tuning of the non-perturbative parameters of those Monte Carlos. These proceedings describe the theoretical advances that have taken place, the impact of the early LHC data, and the areas for future development.

==> MCuncert/text/global.tex <==
%= math ===========================================
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{array}
\usepackage{calc}
\usepackage{longtable}
\usepackage{multirow}
\usepackage{units}
\usepackage{slashed}
%= graphics =======================================
\usepackage{pstricks}
\usepackage{graphicx}
\usepackage{xspace}
%\usepackage{graphpap}
%= citations ======================================
\usepackage{mciteplus}
%= layout =========================================
\usepackage[a4paper,pdfborder={0 0 0}]{hyperref}
\usepackage[format=hang,labelfont=bf,hypcap=true]{caption}
\usepackage{subfig}
\usepackage{sectsty}
\usepackage{placeins}
\allsectionsfont{\sffamily}
\subsubsectionfont{\mdseries\itshape\large}
\setlength{\parindent}{0mm}
\setlength{\hoffset}{-1.75cm}
\setlength{\textwidth}{16.5truecm}
\setlength{\textheight}{24cm}
\setlength{\topmargin}{0mm}
\setlength{\headheight}{0mm}
\setlength{\headsep}{0mm}
\setlength{\parskip}{1mm}
\setlength{\mathindent}{2ex}
\makeatletter
\DeclareRobustCommand*{\bfseries}{%
  \not@math@alphabet\bfseries\mathbf
  \fontseries\bfdefault\selectfont
  \boldmath
}
\makeatother
\let\spreprint\empty
\newcommand{\preprint}[1]{\def\spreprint{\protect#1}}
\let\sinstitute\empty
\newcommand{\institute}[1]{\def\sinstitute{\protect#1}}
\makeatletter
\renewcommand{\maketitle}{\begingroup
  \null\thispagestyle{empty}%
    \ifx\spreprint\empty
      \vskip 5ex
    \else
      \flushright\large\spreprint\vskip 2ex
    \fi
    \vskip 5ex
    \flushleft
      {\sffamily\bfseries\scalebox{0.95}{
	\begin{minipage}{\textwidth}\centering\huge\@title\end{minipage}
      }}\vskip 6ex
      \@author\vskip 2ex
      \ifx\sinstitute\empty
      \else
        {\small\sinstitute}
      \fi
    \vskip 6ex
  \endgroup
}
\makeatother
\renewenvironment{abstract}{\begin{center}
  {\large\sffamily\bfseries Abstract: }
  \begin{minipage}[t]{0.75\textwidth}
}{\end{minipage}\end{center}\vskip 10ex}
\newenvironment{stress}{\vskip 2ex
  \hspace*{2ex}\begin{minipage}{\textwidth-4ex}
  \em}{\end{minipage}\vskip 2ex}
\newcommand{\mytextwidthfigure}[3]{
  \begin{figure}[#1]
    \begin{center}
      #2\\
      \parbox[t]{\textwidth}{\caption{#3}}
    \end{center}
  \end{figure}
}
\newcommand{\myfigure}[3]{
  \begin{figure}[#1]
    \begin{center}
      #2\\
      \parbox[t]{\widthof{#2}}{\caption{#3}}
    \end{center}
  \end{figure}
}
\newcommand{\mytable}[3]{
  \begin{table}[#1]
    \begin{center}
      #2\\
      \parbox[t]{\widthof{#2}}{\caption{#3}}
    \end{center}
  \end{table}
}
%= equation numeration scheme =====================
\numberwithin{equation}{subsection}
%= abbreviations ==================================
% == methods ======================================
\newcommand{\LOPS}{LO$\otimes$PS\xspace}
\newcommand{\NLOPS}{NLO$\otimes$PS\xspace}
\newcommand{\MEPS}{M\protect\scalebox{0.8}{E}P\protect\scalebox{0.8}{S}\xspace}
\newcommand{\MENLOPS}{M\protect\scalebox{0.8}{E}N\protect\scalebox{0.8}{LO}P\protect\scalebox{0.8}{S}\xspace}
\newcommand{\MCatNLO}{M\protect\scalebox{0.8}{C}@N\protect\scalebox{0.8}{LO}\xspace}
\newcommand{\POWHEG}{P\protect\scalebox{0.8}{OWHEG}\xspace}
% == full MC codes ===============================
\newcommand{\aMCatNLO}{aM\protect\scalebox{0.8}{C}@N\protect\scalebox{0.8}{LO}\xspace}
\newcommand{\Ariadne}{A\protect\scalebox{0.8}{RIADNE}\xspace}
\newcommand{\Herwig}{H\protect\scalebox{0.8}{ERWIG}\xspace}
\newcommand{\Herwigpp}{H\protect\scalebox{0.8}{ERWIG++}\xspace}
\newcommand{\Jetset}{J\protect\scalebox{0.8}{ETSET}\xspace}
\newcommand{\PowhegBox}{P\protect\scalebox{0.8}{OWHEG} B\protect\scalebox{0.8}{OX}\xspace}
\newcommand{\Pythia}{P\protect\scalebox{0.8}{YTHIA}\xspace}
\newcommand{\PythiaEight}{P\protect\scalebox{0.8}{YTHIA}8\xspace}
\newcommand{\Sherpa}{S\protect\scalebox{0.8}{HERPA}\xspace}
% == ME codes ==================================
\newcommand{\Alpgen}{A\protect\scalebox{0.8}{LPGEN}\xspace}
\newcommand{\Amegic}{A\protect\scalebox{0.8}{MEGIC++}\xspace}
\newcommand{\BlackHat}{B\protect\scalebox{0.8}{LACK}H\protect\scalebox{0.8}{AT}\xspace}
\newcommand{\Comix}{C\protect\scalebox{0.8}{OMIX}\xspace}
\newcommand{\GoSam}{G\protect\scalebox{0.8}{O}S\protect\scalebox{0.8}{AM}\xspace}
\newcommand{\HEJ}{H\protect\scalebox{0.8}{EJ}\xspace}
\newcommand{\Madevent}{M\protect\scalebox{0.8}{AD}E\protect\scalebox{0.8}{VENT}\xspace}
\newcommand{\Madgraph}{M\protect\scalebox{0.8}{AD}G\protect\scalebox{0.8}{RAPH}\xspace}
\newcommand{\MCFM}{M\protect\scalebox{0.8}{CFM}\xspace}
% == Shower codes ==================================
\newcommand{\Apacic}{A\protect\scalebox{0.8}{PACIC++}\xspace}
\newcommand{\CSS}{C\protect\scalebox{0.8}{SS}\xspace}
\newcommand{\Vincia}{V\protect\scalebox{0.8}{INCIA}\xspace}
% == other codes ==================================
\newcommand{\Diphox}{D\protect\scalebox{0.8}{I}P\protect\scalebox{0.8}{HOX}\xspace}
\newcommand{\FeynRules}{F\protect\scalebox{0.8}{EYN}R\protect\scalebox{0.8}{ULES}\xspace}
\newcommand{\LanHEP}{L\protect\scalebox{0.8}{an}H\protect\scalebox{0.8}{EP}\xspace}
\newcommand{\HqT}{H\protect\scalebox{0.8}{qT}\xspace}
\newcommand{\Jetphox}{J\protect\scalebox{0.8}{ET}P\protect\scalebox{0.8}{HOX}\xspace}
\newcommand{\Professor}{P\protect\scalebox{0.8}{ROFESSOR}\xspace}
\newcommand{\Resbos}{R\protect\scalebox{0.8}{ES}B\protect\scalebox{0.8}{OS}\xspace}
\newcommand{\Rivet}{R\protect\scalebox{0.8}{IVET}\xspace}
\newcommand{\SpringBases}{S\protect\scalebox{0.8}{PRING/}B\protect\scalebox{0.8}{ASES}\xspace}
\newcommand{\Vegas}{V\protect\scalebox{0.8}{EGAS}\xspace}
\newcommand{\Samurai}{S\protect\scalebox{0.8}{AMURAI}\xspace}
\newcommand{\Golem}{golem95\xspace}
% == modules of codes ====================================
\newcommand{\Ahadic}{A\protect\scalebox{0.8}{HADIC++}\xspace}
\newcommand{\Adicic}{A\protect\scalebox{0.8}{DICIC++}\xspace}
\newcommand{\Hadrons}{H\protect\scalebox{0.8}{ADRONS++}\xspace}
\newcommand{\Photons}{P\protect\scalebox{0.8}{HOTONS++}\xspace}
%= experiments etc. ====================================
\newcommand{\Hera}{HERA\xspace}
\newcommand{\LEP}{LEP\xspace}
\newcommand{\LHC}{LHC\xspace}
\newcommand{\Tevatron}{Tevatron\xspace}
\newcommand{\Aleph}{ALEPH\xspace}
\newcommand{\Delphi}{DELPHI\xspace}
\newcommand{\Opal}{OPAL\xspace}
\newcommand{\DO}{D\O\ }
\newcommand{\CDF}{CDF\xspace}
\newcommand{\ATLAS}{ATLAS\xspace}
\newcommand{\CMS}{CMS\xspace}
%= definitions ====================================
\long\def\symbolfootnote[#1]#2{\begingroup%
\def\thefootnote{\fnsymbol{footnote}}\footnote[#1]{#2}\endgroup}
\newcommand{\EqRef}[1]{Eq.~\eqref{#1}}
\newcommand{\EqRefs}[2]{Eqs.~\eqref{#1}-\eqref{#2}}
\newcommand{\SecRef}[1]{Sec.~\ref{#1}}
\newcommand{\FigRef}[1]{Fig.~\ref{#1}}
\newcommand{\FigRefs}[2]{Figs.~\ref{#1}-\ref{#2}}
\newcommand{\TabRef}[1]{Tab.~\ref{#1}}
\newcommand{\TabRefs}[2]{Tabs.~\ref{#1}-\ref{#2}}
\newcommand{\AppRef}[1]{App.~\ref{#1}}

\newcommand{\abs}[1]{\left| #1\right|}
\newcommand{\rbr}[1]{\left( #1\right)}
\newcommand{\abr}[1]{\langle #1\rangle}
\newcommand{\cbr}[1]{\left\{ #1\right\}}
\newcommand{\sbr}[1]{\left[ #1\right]}
\newcommand{\im}{\imath}
\newcommand{\jm}{\jmath}
\newcommand{\ptmin}{p_{\perp,{\rm min}}}
\newcommand{\done}{{\rm d}}
\newcommand{\order}{\mathcal{O}}
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\mr}[1]{\mathrm{#1}}
\newcommand{\mb}[1]{\mathbb{#1}}
\newcommand{\dst}{\displaystyle}
\newcommand{\sst}{\scriptstyle}
\newcommand{\nnb}{\nonumber}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\hl}{\vphantom{$\int_A^B$}}
\newcommand{\alphas}{\ensuremath{\alpha_s}\xspace}
%==================================================
\newcommand{\MElevel}{matrix element level\xspace}
\newcommand{\PSlevel}{parton shower level\xspace}
\newcommand{\Hadlevel}{hadron level\xspace}
\newcommand{\UElevel}{hadron level including UE\xspace}
\newcommand{\QEDlevel}{hadron level including UE and QED final state radiation\xspace}

\newcommand{\todo}[1]{\textbf{\color{red}To do: #1}}
\newcommand{\note}[1]{\textbf{\color{red}Note: #1}}


==> NNPDFewk/NNPDFewk_bib.tex <==
\providecommand{\href}[2]{#2}\begingroup\raggedright\begin{thebibliography}{10}

\bibitem{CMS:2011mea}
S.~Chatrchyan {\em et.~al}, {\bf CMS} Collaboration {\em Phys.Rev.Lett.} {\bf
  107} (2011) 132001, [\href{http://xxx.lanl.gov/abs/1106.0208}{{\tt
  1106.0208}}].

\bibitem{Chatrchyan:2011qta}
S.~Chatrchyan {\em et.~al}, {\bf CMS} Collaboration {\em Phys.Lett.} {\bf
  B700} (2011) 187--206, [\href{http://xxx.lanl.gov/abs/1104.1693}{{\tt
  1104.1693}}].

\bibitem{Collaboration:2011fc}
G.~Aad {\em et.~al}, {\bf ATLAS} Collaboration
  \href{http://xxx.lanl.gov/abs/1112.6297}{{\tt 1112.6297}}.

\bibitem{Aad:2011dm}
G.~Aad {\em et.~al}, {\bf ATLAS} Collaboration
  \href{http://xxx.lanl.gov/abs/1109.5141}{{\tt 1109.5141}}.

\bibitem{Aad:2011yn}
G.~Aad {\em et.~al}, {\bf ATLAS} Collaboration {\em Phys.Lett.} {\bf B701}
  (2011) 31--49, [\href{http://xxx.lanl.gov/abs/1103.2929}{{\tt 1103.2929}}].

\bibitem{CMS234}
{\bf CMS} Collaboration \href{http://xxx.lanl.gov/abs/CMS-PAS-EWK-11-005}{{\tt
  CMS-PAS-EWK-11-005}}.

\bibitem{Chatrchyan:2011jz}
S.~Chatrchyan {\em et.~al}, {\bf CMS} Collaboration {\em JHEP} {\bf 04}
  (2011) 050, [\href{http://xxx.lanl.gov/abs/1103.3470}{{\tt 1103.3470}}].

\bibitem{Chatrchyan:2011wt}
S.~Chatrchyan {\em et.~al}, {\bf CMS} Collaboration
  \href{http://xxx.lanl.gov/abs/1110.4973}{{\tt 1110.4973}}.

\bibitem{LHCb}
{\bf LHCb} Collaboration \href{http://xxx.lanl.gov/abs/LHCb-CONF-2011-039}{{\tt
  LHCb-CONF-2011-039}}.

\bibitem{CMSWc}
{\bf CMS} Collaboration \href{http://xxx.lanl.gov/abs/CMS-PAS-EWK-11-013}{{\tt
  CMS-PAS-EWK-11-013}}.

\bibitem{Aad:2011tw}
G.~Aad {\em et.~al}, {\bf ATLAS} Collaboration {\em Phys. Lett. B} {\bf 706}
  (2011) 150--167, [\href{http://xxx.lanl.gov/abs/1108.0253}{{\tt 1108.0253}}].

\bibitem{Chatrchyan:2011ue}
S.~Chatrchyan {\em et.~al}, {\bf CMS} Collaboration {\em Phys.Rev.} {\bf D84}
  (2011) 052011, [\href{http://xxx.lanl.gov/abs/1108.2044}{{\tt 1108.2044}}].

\bibitem{Ball:2011us}
R.~D. Ball{\em et.~al},
  {\bf NNPDF} Collaboration {\em Phys.Lett.} {\bf B707} (2012) 66--71,
  [\href{http://xxx.lanl.gov/abs/1110.2483}{{\tt 1110.2483}}].

\bibitem{Lionetti:2011pw}
S.~Lionetti {\em et.~al}, {\bf NNPDF} Collaboration {\em Phys. Lett.} {\bf
  B701} (2011) 346--352, [\href{http://xxx.lanl.gov/abs/1103.2369}{{\tt
  1103.2369}}].

\bibitem{Carli:2010rw}
T.~Carli {\em
  et.~al}, {\em Eur.Phys.J.} {\bf C66} (2010) 503--524,
  [\href{http://xxx.lanl.gov/abs/0911.2985}{{\tt 0911.2985}}].

\bibitem{DDE}
D.~D'Enterria and J.~Rojo,. in preparation.

\bibitem{DelDebbio:2004qj}
L.~Del~Debbio {\em et.~al}, {\bf NNPDF} Collaboration {\em JHEP} {\bf 03} (2005) 080,
  [\href{http://xxx.lanl.gov/abs/hep-ph/0501067}{{\tt hep-ph/0501067}}].

\bibitem{DelDebbio:2007ee}
L.~Del~Debbio {\em et.~al}, {\bf NNPDF} Collaboration {\em JHEP} {\bf 03} (2007) 039,
  [\href{http://xxx.lanl.gov/abs/hep-ph/0701127}{{\tt hep-ph/0701127}}].

\bibitem{Ball:2008by}
R.~D. Ball {\em et.~al}, {\bf NNPDF} Collaboration {\em Nucl. Phys.} {\bf
  B809} (2009) 1--63, [\href{http://xxx.lanl.gov/abs/0808.1231}{{\tt
  0808.1231}}].

\bibitem{Ball:2009mk}
R.~D. Ball {\em et.~al}, {\bf NNPDF} Collaboration {\em Nucl. Phys.} {\bf
  B823} (2009) 195--233, [\href{http://xxx.lanl.gov/abs/0906.1958}{{\tt
  0906.1958}}].

\bibitem{Ball:2010de}
R.~D. Ball {\em et.~al}, {\bf {NNPDF}} Collaboration {\em Nucl. Phys.}
  {\bf B838} (2010) 136--206, [\href{http://xxx.lanl.gov/abs/1002.4407}{{\tt
  1002.4407}}].

\bibitem{Ball:2011mu}
R.~D. Ball {\em et.~al}, {\bf NNPDF} Collaboration {\em Nucl. Phys.} {\bf
  B849} (2011) 296--363, [\href{http://xxx.lanl.gov/abs/1101.1300}{{\tt
  1101.1300}}].

\bibitem{Ball:2011uy}
R.~D. Ball {\em et.~al}, {\bf NNPDF} Collaboration {\em Nucl.Phys.} {\bf
  B855} (2012) 153--221, [\href{http://xxx.lanl.gov/abs/1107.2652}{{\tt
  1107.2652}}].

\bibitem{Ball:2011gg}
R.~D. Ball {\em et.~al},
  {\bf NNPDF} Collaboration {\em Nucl.Phys.} {\bf B855} (2012) 608--638,
  [\href{http://xxx.lanl.gov/abs/1108.1758}{{\tt 1108.1758}}].

\bibitem{Catani:2009sm}
S.~Catani {\em et.~al}, {\em Phys.
  Rev. Lett.} {\bf 103} (2009) 082001,
  [\href{http://xxx.lanl.gov/abs/0903.2120}{{\tt 0903.2120}}].

\bibitem{Ball:2010gb}
R.~D. Ball {\em et.~al}, {\bf NNPDF} Collaboration {\em Nucl. Phys.} {\bf
  B849} (2011) 112--143, [\href{http://xxx.lanl.gov/abs/1012.0836}{{\tt
  1012.0836}}].

\bibitem{Martin:2009iq}
A.~D. Martin, W.~J. Stirling, R.~S. Thorne, and G.~Watt, {\em Eur. Phys. J.}
  {\bf C63} (2009) 189--285, [\href{http://xxx.lanl.gov/abs/0901.0002}{{\tt
  0901.0002}}].

\bibitem{Alekhin:2009ni}
S.~Alekhin, J.~Blumlein, S.~Klein, and S.~Moch, {\em Phys. Rev.} {\bf D81}
  (2010) 014032, [\href{http://xxx.lanl.gov/abs/0908.2766}{{\tt 0908.2766}}].

\bibitem{herapdf15}
{\bf H1 and ZEUS} Collaboration. H1prelim-11-042, ZEUS-prel-11-002.

\bibitem{JimenezDelgado:2009tv}
P.~Jimenez-Delgado and E.~Reya, {\em Phys. Rev.} {\bf D80} (2009) 114011,
  [\href{http://xxx.lanl.gov/abs/0909.1711}{{\tt 0909.1711}}].

\bibitem{Ball:2009qv}
R.~D. Ball {\em et.~al}, {\bf NNPDF} Collaboration {\em JHEP} {\bf 05}
  (2010) 075, [\href{http://xxx.lanl.gov/abs/0912.2276}{{\tt 0912.2276}}].

\end{thebibliography}\endgroup


==> Photons/isolationcomplications.tex <==


\subsection{Complications}

Two main differences between experimental conditions and that of theory are
discussed here: the smallest cone and pile-up/underlying event. The Frixione
cone calculation used above assumes that the energy in the final cone can be
calculated, i.e. within a cone of 0.1. However experimentally this isn't
possible, due to the granularity of the detectors and the spread in the shower
of the photon itself. To rectify this the Frixione calculation could be modified
into a `crown' isolation, whereby the last cone is missed from the calculation.
Unfortunately as most of the radiation is collinear in the fragmentation events,
it is likely to reduce its effect of removing these events. The alternative is
to hope that the identification selection used experimentally removes all of
these events and the original Frixione form can be used. Unfortunately
preliminary studies suggest that the selection efficiency is low in events with
collinear radiation, but not zero as hoped~\cite{MartinPrivate}.

As Jetphox is calculated at the parton level it misses the effects from
underlying event (from the remainder of the colliding protons) or from pile-up
(from other proton collisions, either in the same or preceding bunch crossings).
This means that either the experimental isolation has to be corrected before the
isolation criteria can be applied, or the theoretical cross section has to be
corrected to account for this being missed.

Within the ATLAS collaboration this correction is achieved by applying the
technique of jet area corrections~\cite{Cacciari:area,Cacciari:UE}. Details 
of its use in the inclusive cross section measurement are 
in~\cite{InclusivePaper2010}. The ATLAS isolation definition uses a cone
around the cluster of cells that are identified as a photon. These photon cluster
cells are not included in the sum, so there is first a correction for any leakage
of the photon shower into the surrounding cells (typically a few percent of the 
photon $p_T$). The pile-up/underlying event correction is then applied by 
calculating per event the ambient energy from the jet activity in that specific 
event. This follows the jet area corrections method mentioned above, where all
jets are reconstructed without any minimum momentum threshold. The energy density 
of each jet is calculated and the median density is used for the correction.
In 2010 this typically resulted in a correction of around $900 \rm{MeV}$. 

%***Add details of CMS isolation correction here



==> introduction/IntroOld.tex <==
%\documentclass[11pt]{cernrep}
%\usepackage{graphicx,epsfig}
%\bibliographystyle{lesHouches}

%\begin{document}

%\section{Introduction}                                                          
                                                                                 
The workshop in 2011 was the first for which the long-awaited LHC data (at 7     
TeV) was available                                                               
for analysis and comparison to theory. Even though of limited statistical        
power  compared to the ultimate goals of the LHC, this data accesses             
a very wide kinematic range, and probes regions where multiple scales are        
important. The presence of large scales for some processes, on the TeV level,    
points to the importance of electroweak corrections, which have been             
calculated only for some of the important processes. The first hints of a        
Higgs boson have now been observed. In order to search for signs of              
New Physics, as well as to completely understand the Standard Model at the       
LHC, it is important to                                                          
understand the {\it perturbative framework} at the LHC. The data taken so far    
provides many                                                                    
challenges for perturbative QCD predictions; and it is clear that New            
Physics, if it is present in current data, is hiding well.                              
                                                                                 
On the theoretical side, there has been a great deal of                          
productivity in the area of multi-particle calculations at next-to-leading         
order  (NLO)  and  next-to-next-to-leading order (NNLO).                                            
NLO is the first order at which the normalization,                               
and in some cases the shape, of perturbative cross sections can be considered    
reliable~\cite{Campbell:2006wx}.  A full                                         
understanding for both Standard Model and beyond the Standard Model physics      
at the LHC requires the development of fast, reliable programs for the           
calculation of multi-parton final states at NLO. There have been many            
advances in                                                                      
the development of NLO techniques, especially in the area of                     
automation~\cite{Agrawal:2011tm,Belanger:2003sd,Berger:2008sj,Badger:2010nx,Mastrolia:2010nb,Ellis:2011cr,Hirschi:2011pa,Campbell:2011cu,Bevilacqua:2011xh,Reina:2011mb,Cullen:2011ac}. 

Some of these approaches also allow for
relatively easy~\cite{Alioli:2010xd,Garzelli:2011vp,Cullen:2011ac} and/or
automatic~\cite{Frederix:2011zi} inclusion of the NLO matrix elements into
parton shower Monte Carlo programs.
For more details we refer to the individual contributions in these proceedings.     
                                                                                 
                                                                                 
A prioritized list of NLO (and some NNLO) cross sections was assembled at Les Houches in         
2005~\cite{Buttar:2006zd} and added to in 2007~\cite{Bern:2008ef} and             
2009~\cite{Binoth:2010ra}. This list                                                          
includes cross sections which are experimentally important, and which are        
theoretically feasible (if difficult) to calculate. As we stand now,             
basically all NLO                                                                    
$2\rightarrow 3$  and $2\rightarrow 4$ cross sections of interest have been        
calculated, see Tables~\ref{tab:wishlist1},\ref{tab:wishlist2} below, 
and even some processes which were not on the 2009 wishlist  
are available at NLO, see e.g. 
\cite{Bern:2011ep,Ita:2011wn,Campanario:2011ud,Berger:2010zx,Bevilacqua:2010qb,Dittmaier:2011ti,Denner:2010jp}.
%(with the exception of $t\bar{t}t\bar{t}$ production). 
The success of                                                                               
automation techniques means that future NLO calculations of similar              
complexity can be completed                                                      
without the man-years of labor previously required. Thus, we do not add to       
the NLO wish list in 2011.                                                       
Instead, we comment on calculations needed at NNLO, and processes at NLO for     
which it is important to                                                         
calculate the impact of electroweak corrections, and/or the influence of         
interference effects with                                                        
other processes with the same final state.                                       
                                                                                 
For many of the processes calculated at the LHC (such as for Higgs               
production), it is important either to apply a veto for the production of        
extra jets, or to bin the analysis results according to the jet multiplicity.    
While such cuts are useful for dealing with the experimental backgrounds, the    
exclusivity of the cross sections results in increases to the theoretical        
uncertainties obtained for the corresponding inclusive results, see e.g.~\cite{Stewart:2011cf} . 
The impact of    
such cuts is explored in the contribution of Stewart and Tackmann in these proceedings.               
                                                                                                                                                                  
%Table{bel{tab:wishlist}}                                                        
\begin{table}                                                                    
  \begin{center}                                                                 
     \begin{tabular}{|l|l|}                                                      
\hline \hline                                                                    
Process ($V\in\{Z,W,\gamma\}$) & Comments\\                                      
\hline                                                                           
Calculations completed since Les Houches 2005&\\                                 
\hline                                                                           
&\\                                                                              
1. $pp\to VV$\,jet & $WW$\,jet completed by                                          
Dittmaier/Kallweit/Uwer~\cite{Dittmaier:2007th,Dittmaier:2009un};\\              
 &                                                                               
Campbell/Ellis/Zanderighi~\cite{Campbell:2007ev}.\\                              
 &                                                                               
$ZZ$jet completed by \\                                                          
&                                                                                
Binoth/Gleisberg/Karg/Kauer/Sanguinetti~\cite{Binoth:2009wk}\\                   
%and Binoth/Karg/Kauer/Sanguinetti (in progress)\\                               
2. $pp \to$ Higgs+2jets & NLO QCD to the $gg$ channel \\                         
& completed by Campbell/Ellis/Zanderighi~\cite{Campbell:2006xx};\\               
& NLO QCD+EW to the VBF channel\\                                                
& completed by                                                                   
Ciccolini/Denner/Dittmaier~\cite{Ciccolini:2007jr,Ciccolini:2007ec} \\ 
& Interference QCD-EW in VBF channel~\cite{Andersen:2007mp,Bredenstein:2008tm} \\          
3. $pp\to V\,V\,V$ & $ZZZ$ completed                                             
by Lazopoulos/Melnikov/Petriello~\cite{Lazopoulos:2007ix}                        
 \\                                                                              
 & and $WWZ$ by Hankele/Zeppenfeld~\cite{Hankele:2007sb},\\                       
 & see also Binoth/Ossola/Papadopoulos/Pittau~\cite{Binoth:2008kt}  \\ 
 & VBFNLO~\cite{Arnold:2011wj,Campanario:2011fs} meanwhile also contains  \\
 & $WWW,ZZW,WW\gamma,ZZ\gamma,WZ\gamma,W\gamma\gamma,Z\gamma\gamma,\gamma\gamma\gamma$\\    
&$WZj,W\gamma j,\gamma j j, W\gamma \gamma j $\\                                                                              
&\\                                                                              
4. $pp\to t\bar{t}\,b\bar{b}$ &  relevant for $t\bar{t}H$, computed by\\          
 &                                                                               
Bredenstein/Denner/Dittmaier/Pozzorini~\cite{Bredenstein:2009aj,Bredenstein:2010rs} \\                                                                        
 & and Bevilacqua/Czakon/Papadopoulos/Pittau/Worek~\cite{Bevilacqua:2009zn}      
\\                                                                               
5. $pp \to V$+3jets & $W$+3jets calculated by the Blackhat/Sherpa~\cite{Berger:2009ep}     
\\                                                                               
 & and Rocket~\cite{Ellis:2009zw} collaborations\\ 
 &$Z$+3jets  by Blackhat/Sherpa~\cite{Berger:2010vm}  \\                                                                                                   
 \hline                                                                          
Calculations remaining from Les Houches 2005&\\                                  
\hline                                                                           
&\\                                                                              
6. $pp\to t\bar{t}$+2jets & relevant for $t\bar{t}H$, computed by  \\             
& Bevilacqua/Czakon/Papadopoulos/Worek                                           
~\cite{Bevilacqua:2010ve,Bevilacqua:2011aa}                                                        
\\                                                                               
7. $pp\to VV\,b\bar{b}$, & Pozzorini et al.\cite{Denner:2010jp},Bevilacqua et
al.\cite{Bevilacqua:2010qb}  \\
%relevant for VBF $\rightarrow H\rightarrow   VV$,~$t\bar{t}H$ \\                                                              
8. $pp\to VV$+2jets  & $W^+W^+$+2jets~\cite{Melia:2010bm},
$W^+W^-$+2jets~\cite{Melia:2011dw,Greiner:2012im},  \\
%relevant for VBF $\rightarrow H\rightarrow VV$ \\         
& VBF contributions calculated by \\                                             
& (Bozzi/)J\"ager/Oleari/Zeppenfeld~\cite{Jager:2006zc,Jager:2006cp,Bozzi:2007ur}                                                                               
\\                                                                               
\hline                                                                           
NLO calculations added to list in 2007&\\                                        
\hline                                                                           
&\\                                                                              
9. $pp\to b\bar{b}b\bar{b}$ &Binoth et al.~\cite{Binoth:2009rv,Greiner:2011mp} \\                                            
&\\                                                                              
%10. $pp\to 4$jets &  \\                                                         
\hline                                                                           
NLO calculations added to list in 2009&\\                                        
\hline                                                                           
&\\                                                                              
10. $pp \to V$\,+\,4 jets & top pair production, various new physics signatures\\ 
& Blackhat/Sherpa: $W$+4jets~\cite{Berger:2010zx},  $Z$+4jets~\cite{Ita:2011wn} \\
& see also HEJ~\cite{Andersen:2011hs} for $W+n$jets\\
11. $pp \to W b \bar{b}j$ & top, new physics signatures,  
 Reina/Schutzmeier~\cite{Reina:2011mb}\\                      
12. $pp \to t\bar{t}t\bar{t}$ & various new physics signatures \\
&\\   
also: $pp\to $ 4\,jets &   Blackhat/Sherpa~\cite{Bern:2011ep}  \\  
&\\       
\hline 
\end{tabular}
\end{center}
\caption{The updated experimenter's wishlist for LHC processes                   
\label{tab:wishlist1}}                                                            
\end{table} 

\begin{table}                                                                    
  \begin{center}                                                                 
     \begin{tabular}{|l|l|}                                                      
\hline                                                                   
Calculations beyond NLO added in 2007&\\                                         
\hline                                                                           
&\\                                                                              
13. $gg\to W^*W^*$ ${\cal O}(\alpha^2\alpha_s^3)$& backgrounds to Higgs\\        
14. NNLO $pp\to t\bar{t}$ & normalization of a benchmark process\\               
15. NNLO to VBF and $Z/\gamma$+jet  & Higgs couplings and SM benchmark\\ 
&\\                                                                                     
\hline                                                                           
Calculations including electroweak effects&\\                                    
\hline                                                                           
&\\                                                                              
16. NNLO QCD+NLO EW for $W/Z$ & precision calculation of a SM benchmark\\
NLO EW to $W/Z$ &\cite{Kuhn:2007cv,Hollik:2007sq}\\
NLO EW to $W/Z$+jet&\cite{Denner:2009gj,Denner:2011vu}\\ 
NLO EW to $WH/ZH$ &\cite{Denner:2011id}\\       
&\\                                                                              
\hline                                                                           
\hline                                                                           
\end{tabular}                                                                    
\end{center}                                                                     
\caption{The updated experimenter's wishlist for LHC processes continued                  
\label{tab:wishlist2}}                                                            
\end{table}                                                                      
                                                                                  
Much of the complexity for multi-parton NLO processes consists of the            
calculation of the non-leading color contributions. Such contributions           
typically contribute only at the level of a few percent 
%{\it do we know how this may scale with increasing  number of partons? }                  
and approximations to the non-leading color contributions should be accurate     
within a percent or so~\cite{Berger:2009zg,Melnikov:2009wh,Berger:2009ep}. 
So it may be more time-prudent for groups carrying out such calculations to estimate the           
non-leading color effects before carrying out the full calculation.       
                                                                                 
To reach full utility, the codes for any of these                                
complex NLO calculations should be made public and/or the authors should         
generate \textsc{ROOT} ntuples                                                            
providing the parton level event information from which experimentalists         
can assemble any cross sections of interest. Where possible, decays (with        
spin correlations) should be included. A \textsc{ROOT} output option is especially        
useful where the creation of a user-friendly NLO program may be very             
time-consuming.                                                                  
We now have some experience with the use of \textsc{ROOT} ntuples with both MCFM and      
Blackhat+Sherpa calculations.                                                    
%{\it what other programs use \textsc{ROOT} tuples as output? 
%GoSam+Sherpa produces RIVET output}                                 
 The latter, in particular, does not exist as a public program, while \textsc{ROOT}       
tuples have been made available for NLO W/Z + n jet multiplicities (with n up    
to 4) for W/Z + jets, and (also for n up to 4) for inclusive jet production.     
The estimation of the {\it correct} scale for use in multi-parton NLO            
calculations, and the proper evaluation of the uncertainty on this scale, is     
more complex than for simpler calculations. The use of \textsc{ROOT} ntuples can make     
these evaluations easier to carry out.                                           
A contribution describing their use has been included in these proceedings.      
                                                                                 
While NLO is sufficient for most predictions,  it is also crucial to             
understand certain critical cross sections at NNLO. To date, NNLO                
calculations have been carried out primarily for  
processes in $e^+e^-$ annihilation~\cite{GehrmannDeRidder:2007hr,GehrmannDeRidder:2008ug,Weinzierl:2009ms}, 
and in hadronic collisions for $2\rightarrow 1$ processes,        
with the exception of VH~\cite{Brein:2003wg,Brein:2011vx,Ferrera:2011bk} 
and $\gamma\gamma$ production~\cite{Catani:2011qz}. 

To calculate a $2\to 2$ scattering process at NNLO, 
the divergent contributions arising from the              
tree-level $2\rightarrow 4$, the one-loop $2\rightarrow 3$            
and the two-loop $2\rightarrow 2$ subprocesses have to be 
properly subtracted and cancelled, such that the finite remainders 
can be combined into a parton-level event generator. 
To combine the three contributions, an infra-red subtraction scheme 
for unresolved real radiation is required.   
Several approaches have been used and are being further developed:
antenna subtraction~\cite{GehrmannDeRidder:2005cm}, 
which currently is extended to hadronic and semi-hadronic 
initial
states~\cite{Daleo:2009yj,Gehrmann:2009vu,Gehrmann:2011wi,Abelof:2011jv,Boughezal:2010mc}, 
a method based on sector decomposition appplied to 
real radiation~\cite{Heinrich:2002rc,Anastasiou:2003gr,Binoth:2004jv} 
where the decomposition is guided by the physical 
singularity structure~\cite{Czakon:2010td,Boughezal:2011jf}, 
$q_T$-subtraction~\cite{Catani:2007vq}, which is very elegant but appplicable only to 
colourless final states, and the one of \cite{Bolzoni:2010bt} described in these proceedings.


Further, two-loop amplitudes are interesting in     
their own right from a field theory point of view, 
for example to study asymptotic behaviour, or to 
gain insights into the all-order infared structure of massless 
field theories. 

Below we construct a table of calculations needed at the LHC, and which are      
feasible within the next few years.                                              
Certainly, results for  inclusive cross sections at NNLO will be 
easier to achieve than  differential distributions, 
but most groups are working towards a partonic Monte Carlo program 
capable of producing fully differential distributions for measured observables.
                                                                                 
\begin{itemize}    
\item $t\bar{t}$ production:\\  
needed for accurate background estimates, top mass measurement, 
top quark asymmetry  (which is zero at tree level, so NLO is the 
leading non-vanishing order for this observable, and a discrepancy 
of theory predictions with Tevatron data 
needs to be understood).  Several groups are already well on the way to 
complete NNLO results for $t\bar{t}$
production~\cite{Bonciani:2010mn,Abelof:2011ap,Czakon:2011ve,Czakon:2011xx}.


\item $W^+W^-$ production:\\
importand background to Higgs search. 
At the LHC, $gg\to WW$ is the dominant subprocess, but
$gg\to WW$ is a loop-induced process, such that two loops 
need to be calculated to get a reliable estimate of the cross section. 
Advances towards the full two-loop result are 
reported in~\cite{Chachamis:2010zz,Chachamis:2008yb}.                                                                       

\item inclusive jet/dijet production:\\
NNLO parton distribution function (PDF) fits are starting to become the norm     
for predictions and comparisons at the LHC. Paramount in these global fits is the    
use of inclusive jet production to tie down the behavior of the gluon            
distribution, especially at high $x$. However, while the other essential         
processes used in the global fitting are known to NNLO, the inclusive jet        
production cross section is only known at NLO. Thus, it is crucial for           
precision predictions for the LHC for the NNLO corrections for this process      
to be calculated, and to be available for inclusion in the global PDF fits. 
First results for the real-virtual and double real corrections to 
gluon scattering 
can be found in~\cite{GehrmannDeRidder:2011aa,Pires:2010jv}.     
                                                                                 
\item V+1 jet production:\\  
$W/Z/\gamma$ + jet production form the signal channels (and backgrounds) for     
many key physics processes, for both SM and BSM. In addition, they also serve    
as calibration tools for the jet energy scale and for the crucial                
understanding of the missing transverse energy resolution.  
The two-loop amplitudes for this process are
known~\cite{Garland:2001tf,Garland:2002ak}, 
therefore it can be calculated once the parts involving unresolved real
radiation are available.

\item V+$\gamma$ production:\\
important signal/background processes for Higgs and New Physics searches.
The two-loop helicity amplitudes for 
$q\bar q \to W^\pm \gamma$ and $q\bar q \to Z^0 \gamma$  
recently have become available~\cite{Gehrmann:2011ab}.                   
                                                                                 
\item Higgs+1 jet production:\\  
As mentioned previously, events in many of the experimental Higgs analyses       
are separated by the number of additional jets accompanying the Higgs boson.     
In many searches, the Higgs + 0 jet and Higgs + 1 jet bins contribute            
approximately equally to the sensitivity. It is thus necessary to have the       
same theoretical accuracy for the Higgs + 1 jet cross section as already         
exists for the inclusive Higgs cross section, i.e. NNLO.  
The two-Loop QCD Corrections to the Helicity Amplitudes for
$H \to$ 3 partons are already available~\cite{Gehrmann:2011aa}.
\end{itemize}                     
                                                                                 
The contributions in this document are arranged as follows.
In section~\ref{part:nlo}, various developments concerning techniques for NLO and NNLO calculations are described, in particular in view of
providing automated tools for NLO corrections.
In section~\ref{part:pdf}, issues related to parton distribution functions are discussed. Section ~\ref{part:pheno} contains phenomenological studies
of observables and uncertainties, based on theory input where
higher order corrections obtained by different approaches are available.
Section~\ref{part:corr} includes phenomenological studies on the definition of experimental observables and corrections applied to data.
Finally Section~\ref{part:mc} discusses issues related to the tuning of Monte Carlos and standardised Monte Carlo output formats.

%\bibliography{LH11}

                                                                                 
%\end{document} 

